Towards standardizing Korean Grammatical Error Correction: Datasets and Annotation

Research on Korean grammatical error correction (GEC) is limited, compared to other major languages such as English. We attribute this problematic circumstance to the lack of a carefully designed evaluation benchmark for Korean GEC. In this work, we collect three datasets from different sources (Kor-Lang8, Kor-Native, and Kor-Learner) that covers a wide range of Korean grammatical errors. Considering the nature of Korean grammar, We then define 14 error types for Korean and provide KAGAS (Korean Automatic Grammatical error Annotation System), which can automatically annotate error types from parallel corpora. We use KAGAS on our datasets to make an evaluation benchmark for Korean, and present baseline models trained from our datasets. We show that the model trained with our datasets significantly outperforms the currently used statistical Korean GEC system (Hanspell) on a wider range of error types, demonstrating the diversity and usefulness of the datasets. The implementations and datasets are open-sourced.

==> 025_korean_language.tex <==
\section{Korean Language}
\label{sec:korean_language}
write in high-level (with keyword and examples) about the differences between Korean and English

Korean is agglutinative, so low probability that insertion and deletion happen 
- 한국어 writing 에서 틀릴 수 있는 에러 정리
- 영어와 어떻게 다른지
- WS가 뭔지, 무슨 뜻인지, agglutinative, native speaker와 korean learner가 왜 틀리는지

==> figs/denoised_heatmap.tex <==
\begin{figure}[!h]
{
\includegraphics[width=\linewidth]{imgs/denoised_heatmap.png}
}
\caption{Heatmap illustration of error types generated by Denoising. }
\label{fig:denoised_heatmap}
\end{figure}


==> figs/eval_demos.tex <==
\begin{figure}[!h]
\centering
\includegraphics[width=\linewidth]{imgs/kagas_eval.png}
\label{fig:eval_demos}
\caption{Website that we used for KAGAS system evaluation. Translated into english.}
\end{figure}


==> figs/hanspell_heatmap.tex <==
\begin{figure}[!h]
{
\includegraphics[width=\linewidth]{imgs/hanspell_heatmap.png}
}
\caption{Heatmap illustration of error types generated by the Hanspell library. }
\label{fig:hanspell_heatmap}
\end{figure}


==> figs/kobart_heatmap.tex <==
\begin{figure}[!h]
{
\includegraphics[width=\linewidth]{imgs/kobart_heatmap.png}
}
\caption{Heatmap illustration of error types generated by finetuning on top of KoBART. }
\label{fig:kobart_heatmap}
\end{figure}


==> tabs/kagas_errortypes.tex <==
\begin{table}[ht]
\small
\centering
\begin{tabularx}{\linewidth}{lXr}
\toprule
  Code &
  Description &
  \makecell{Acceptance \\ Rate (\%)} \\
\midrule
  
  INS &
  A word is inserted. &
  100.00 ± 0.00 \\
   
  DEL &
  A word is deleted. &
  100.00 ± 0.00 \\
  
  WS &
  Spacing between words is changed. &
  100.00 ± 0.00 \\
  
  WO &
  Word order is changed. &
  96.15 ± 0.07 \\
  
  SPELL &
  Spelling error &
  96.15 ± 0.07 \\
  
  PUNCT &
  Punctuation error &
  100.00 ± 0.00 \\
  
  SHORT &
  {An edit that does not change the structure of morphemes.} &
  69.23 ± 0.18 \\
  
  VERB &
  An error on verb &
  65.38 ± 0.18 \\

  ADJ &
  An error on adjective &
  69.23 ± 0.18 \\

  NOUN &
  An error on noun &
  69.23 ± 0.18 \\

  PART &
  An error on particle &
  96.15 ± 0.07 \\

  END &
  An error on ending &
  80.77 ± 0.15 \\

  MOD &
  An error on modifier &
  92.31 ± 0.10 \\

  CONJ &
  An error on conjugation &
  42.31 ± 0.19 \\
  
  \bottomrule
\end{tabularx}
\caption{Full category of error types that KAGAS use. }
\label{tabs:kagas_errortypes}
\end{table}

==> tabs/kagas_errortypes_backup.tex <==
\begin{table}[ht]
\small
\centering
\begin{tabularx}{\linewidth}{lXXr}
\toprule
  Code &
  Description &
  Example &
  \makecell{Acceptance \\ Rate (\%)} \\
\midrule
  
  INS &
  A word is inserted. &
  \makecell{$\emptyset$\\->규칙을}&
  \makecell{\tiny100.00 ± 0.00} \\
   
  DEL &
  A word is deleted. &
  \makecell{끝 \\->$\emptyset$} &
  \makecell{\tiny100.00 ± 0.00} \\
  
  WS &
  Spacing between words is changed. &
   \makecell{이옷은\\->이 옷은} &
   \makecell{\tiny100.00 ± 0.00} \\
  
  WO &
  Word order is changed. &
  \makecell{\tiny더 한국어를\\-> 한국어를 더} &
  \makecell{\tiny96.15 ± 0.07} \\
  
  SPELL &
  Spelling error &
   \makecell{쳐요\\->춰요} &
   \makecell{\tiny96.15 ± 0.07} \\
  
  PUNCT &
  Punctuation error &
  \makecell{의\\->,} &
  \makecell{\tiny100.00 ± 0.00} \\
  
  SHORT &
  {Reorganizes the structure of morphemes.} &
  \makecell{이었\\->였} &
  \makecell{\tiny69.23 ± 0.18} \\
  
  VERB &
  An error on verb &
   \makecell{쌌어요\\->썼어요} &
  \makecell{\tiny65.38 ± 0.18} \\

  ADJ &
  An error on adjective &
  \makecell{진한\\->친한} &
 \makecell{\tiny69.23 ± 0.18} \\

  NOUN &
  An error on noun &
  \makecell{유학러\\->유학} &
  \makecell{\tiny69.23 ± 0.18} \\

  PART &
  An error on particle &
  \makecell{에서\\-> 에} &
  \makecell{\tiny96.15 ± 0.07} \\

  END &
  An error on ending &
  \makecell{려요\\->렸어요} &
  \makecell{\tiny80.77 ± 0.15} \\

  MOD &
  An error on modifier &
  \makecell{나무\\-> 너무} &
 \makecell{\tiny92.31 ± 0.10} \\

  CONJ &
  An error on conjugation &
  \makecell{잘라에\\-> 자르러} &
  \makecell{\tiny42.31 ± 0.19} \\
  
  \bottomrule
\end{tabularx}
\caption{Full category of error types that KAGAS use.}
\label{tabs:kagas_errortypes}
\end{table}

==> tabs/kagas_errortypes_one_column.tex <==
\begin{table*}[ht]
\centering
\begin{tabular}{ll|r}
\toprule
  Error type code &
  Description &
  Acceptance Rate \\
\midrule
  
  INS &
  A word is inserted. &
  100.00\% ± 0.00\%P \\
   
  DEL &
  A word is deleted. &
  100.00\% ± 0.00\%P \\
  
  WS &
  Spacing between words is changed. &
  100.00\% ± 0.00\%P \\
  
  WO &
  The order of words is changed. &
  97.44\% ± 3.51\%P \\
  
  SPELL &
  Spelling error &
  97.44\% ± 3.51\%P \\
  
  PUNCT &
  Punctuation error &
  98.72\% ± 2.50\%P \\
  
  SHORT &
  An edit that does not change the structure of morphemes. &
  73.08\% ± 9.84\%P \\
  
  VERB &
  An error on verb &
  79.49\% ± 8.96\%P \\

  ADJ &
  An error on adjective &
  73.08\% ± 9.84\%P \\

  NOUN &
  An error on noun &
  75.64\% ± 9.53\%P \\

  PART &
  An error on particle &
  97.44\% ± 3.51\%P \\

  END &
  An error on ending &
  87.18\% ± 7.42\%P \\

  MOD &
  An error on modifier &
  89.74\% ± 6.73\%P \\

  CONJ &
  An error on conjugation &
  43.59\% ± 11.00\%P \\
  
  \bottomrule
\end{tabular}
\caption{Full category of error types used in KAGAS,along with acceptance rates by each error type on human evaluation. }
\end{table*}


==> tabs/kagas_examples.tex <==
\begin{table}
\centering
\resizebox{0.45\textwidth}{!}{
\begin{tabular}{ccccccc}
\multicolumn{7}{l}{\textless{}Korean\textgreater{}} \\
그는 &
  \multicolumn{1}{c|}{방을} &
  \multicolumn{1}{c|}{\textbf{저장한}} &
  \multicolumn{1}{c|}{다음에} &
  \textbf{갔다} &
  \multicolumn{1}{c|}{\textbf{학교에}} &
  . \\
그는 &
  \multicolumn{1}{c|}{방을} &
  \multicolumn{1}{c|}{\textbf{정리한}} &
  \multicolumn{1}{c|}{다음에} &
  \textbf{학교에} &
  \multicolumn{1}{c|}{\textbf{갔다}} &
  . \\
 &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{\textbf{VERB}} &
  \multicolumn{1}{c|}{} &
  \multicolumn{2}{c|}{\textbf{WO(Word Order)}} &
   \\
\multicolumn{7}{l}{} \\
\multicolumn{7}{l}{\textless{}Translated in English\textgreater{}} \\
\multicolumn{1}{c|}{He} & \textbf{to school}  & \multicolumn{1}{c|}{\textbf{went}} & \multicolumn{1}{c|}{after} & \multicolumn{1}{c|}{\textbf{saving}} & his room & . \\
\multicolumn{1}{c|}{He} & \textbf{went} & \multicolumn{1}{c|}{\textbf{to school}}  & \multicolumn{1}{c|}{after} & \multicolumn{1}{c|}{\textbf{cleaning}}  & his room & . \\
\multicolumn{1}{c|}{} &
  \multicolumn{2}{c|}{\textbf{WO(Word Order)}} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{\textbf{VERB}} &
   &
  
\end{tabular}}
\caption{An example visualization on $M^2$ file output of KAGAS given original and corrected sentence pairs. Note that Korean words and English words doesn't necessary align.}
\label{tabs:kagas_examples}
\end{table}

==> tabs/test_valid_errortype_count.tex <==
\begin{table*}[ht]
\centering
\begin{threeparttable}
\resizebox{0.8\textwidth}{!}{
\begin{tabular}{|c|cc|cc|cc|cc|}
\hline
\multirow{2}{*}{Error Type} & \multicolumn{2}{c|}{\klearner{}} & \multicolumn{2}{c|}{\knative{}} & \multicolumn{2}{c|}{\klang{}} & \multicolumn{2}{c|}{\kunion{}} \\
             & valid & test & valid & test & valid & test  & valid & test  \\ \hline
INS    & 450   & 517  & 331   & 304  & 4179  & 4187  & 4960  & 5008  \\
DEL     & 249   & 205  & 94    & 108  & 4131  & 4164  & 4474  & 4477  \\
SPELL        & 828   & 879  & 196   & 156  & 2092  & 2151  & 3116  & 3186  \\
PUNCT        & 0     & 3    & 21    & 12   & 604   & 571   & 625   & 586   \\
SHORT      & 65    & 54   & 34    & 38   & 160   & 136   & 259   & 228   \\
WS           & 19    & 30   & 2336  & 2383 & 1434  & 1440  & 3789  & 3853  \\
WO           & 0     & 0    & 4     & 10   & 95    & 95    & 99    & 105   \\
NOUN         & 785   & 797  & 218   & 208  & 3067  & 3119  & 4070  & 4124  \\
VERB         & 394   & 408  & 74    & 90   & 1350  & 1323  & 1818  & 1821  \\
ADJ    & 77    & 63   & 14    & 15   & 248   & 225   & 339   & 303   \\
CONJ  & 769   & 744  & 312   & 308  & 4863  & 4587  & 5944  & 5639  \\
PART     & 2464  & 3405 & 198   & 176  & 5878  & 6042  & 8540  & 8623  \\
END       & 1084  & 1104 & 92    & 103  & 3367  & 3283  & 4543  & 4490  \\
MOD     & 149   & 163  & 50    & 40   & 792   & 815   & 991   & 1018  \\
UNK & 1483  & 1506 & 633   & 578  & 6486  & 6521  & 8602  & 8605  \\
TOTAL        & 8816  & 8878 & 4607  & 4529 & 38746 & 38659 & 52169 & 52066 \\ \hline
\end{tabular}}
\end{threeparttable}
\caption{Count of occurences of different error type edits from each of the valid dataset. This corresponds to tokenized->detokenized pair from the raw data. We add a valid sentence as each error types if that error type appeared at least once inside the sentence. Therefore, a sentence with multiple error type edits can be counted in duplicate for all of the appeared error types. Therefore the summation of total number for occurences may be larger than the actual validation dataset sentence size.}
\label{tabs:test_valid_errortype_count}
\end{table*}
